Behaviour of electron content in the ionospheric D-region during solar X-ray flares

One of the most important parameters in ionospheric plasma research also having a wide practical application in wireless satellite telecommunications is the total electron content (TEC) representing the columnal electron number density. The F region with high electron density provides the biggest contribution to TEC while the relatively weakly ionized plasma of the D region (60 km - 90 km above Earths surface) is often considered as a negligible cause of satellite signal disturbances. However, sudden intensive ionization processes like those induced by solar X ray flares can cause relative increases of electron density that are significantly larger in the D-region than in regions at higher altitudes. Therefore, one cannot exclude a priori the D region from investigations of ionospheric influences on propagation of electromagnetic signals emitted by satellites. We discuss here this problem which has not been sufficiently treated in literature so far. The obtained results are based on data collected from the D region monitoring by very low frequency radio waves and on vertical TEC calculations from the Global Navigation Satellite System (GNSS) signal analyses, and they show noticeable variations in the D region electron content (TECD) during activity of a solar X ray flare (it rises by a factor of 136 in the considered case) when TECD contribution to TEC can reach several percent and which cannot be neglected in practical applications like global positioning procedures by satellites.

==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.8em{\hfil.\hfil}%
\setbox8=\hbox to0.8em{\hfil$^{#1}$\hfil}%
\box7\kern-0.8em\box8}}

\def\dd{\point{\rm d}}
\def\hh{\point{\rm h}}
\def\mm{\point{\rm m}}
\def\ss{\point{\rm s}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



